RPS: A Generic Reservoir Patterns Sampler

Efficient learning from streaming data is important for modern data analysis due to the continuous and rapid evolution of data streams. Despite significant advancements in stream pattern mining, challenges persist, particularly in managing complex data streams like sequential and weighted itemsets. While reservoir sampling serves as a fundamental method for randomly selecting fixed-size samples from data streams, its application to such complex patterns remains largely unexplored. In this study, we introduce an approach that harnesses a weighted reservoir to facilitate direct pattern sampling from streaming batch data, thus ensuring scalability and efficiency. We present a generic algorithm capable of addressing temporal biases and handling various pattern types, including sequential, weighted, and unweighted itemsets. Through comprehensive experiments conducted on real-world datasets, we evaluate the effectiveness of our method, showcasing its ability to construct accurate incremental online classifiers for sequential data. Our approach not only enables previously unusable online machine learning models for sequential data to achieve accuracy comparable to offline baselines but also represents significant progress in the development of incremental online sequential itemset classifiers.

==> tex/osa.tex <==


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

The overarching goal is to achieve energy-efficient sensor usage and energy conservation in an IoT-based cattle control system through intelligent graph management and sensor activation strategies, thereby contributing to the sustainability and prolonged operation of the IoT network.  The pattern-based energy device monitoring algorithm is described as follows:


\begin{algorithm}
\caption{Pattern-based energy device monitoring}
\label{alg:optimistic_shepherd}
{\small
\begin{algorithmic}[1]
	\Statex \textbf{Input:} A dynamic graph $\dynaGraph(\vertices, \edges_\timestamp)$, a reservoir \reservoir, a minimum \mMinNorm and a maximum \mMaxNorm length constraints
	\State $\timestamp \gets \timestamp_0$, all vertices are active
	\While{$\timestamp > \timestamp_0$}
	\Statex\quad \emph{// Broadcast neighbors at each timestamp as a batch}
	\For{$\vertex_i \in \activeNodes_\timestamp$} %Broadcast neighbors: 
	\State $\instance_i=\{(\vertex, \vertex.\text{batteryLevel}): \vertex \in \neighbors(\vertex_i, \timestamp)\}$
	\State $\vertex.\text{batteryLevel} \gets \vertex.\text{batteryLevel} - E_{\text{basic}}$ for $\vertex \in \neighbors(\vertex_i, \timestamp)$
	\State Send $\instance_i$ to local system
	\State $\vertex_i.\text{batteryLevel} \gets \vertex_i.\text{batteryLevel} - E_{\text{payload}}(\vertex_i, \timestamp)$
	\EndFor
	\Statex\quad \emph{// Recover the set of instances as a batch}
	\State Let $\batch$ be the set of instances of neighbors sent in line 4
	\If{\card{\batch}>0}
	\State $\reservoir\gets \myalgodampedwindow(\reservoir, (\timestamp, \batch), (\damping, \dampingFactor), \reservoirSize, (\mUtility)\times(\mMinNorm) \times(\mMaxNorm))$
	\Statex\quad\quad\quad \emph{// Set vertices in passive mode based on trust patterns}
	\For{$\vertex \in \vertices$}
	\If{$\vertex.getBatteryLevel()>0$}
	\If{freq($\vertex, \reservoir) \geq 2$}
	\State $\vertex.STATUS \gets PASSIVE$
	\Else ~$\vertex.STATUS \gets ACTIVE$
	\EndIf
	\ElsIf{$\vertex.STATUS \neq OFF$} 
	\State $\vertex.STATUS \gets OFF$
	\EndIf
	\EndFor
	\Else \emph{ // The system is in an idle state and should be woken up}
	\ForAll{$\vertex \in \passiveNodes_\timestamp$}
	\If{$\vertex.getBatteryLevel()>0$}
	\State $\vertex.STATUS \gets ACTIVE$
	\ElsIf{$\vertex.STATUS \neq OFF$} 
	\State $\vertex.STATUS \gets OFF$
	\EndIf
	\EndFor
	\EndIf
	\State $\timestamp \gets Next(timestamp)$
	\EndWhile
\end{algorithmic}
}
\end{algorithm}


The algorithm operates in a loop where each iteration corresponds to a timestamp in the dynamic graph. At each timestamp, the active nodes broadcast information about their neighbors, including battery levels, to a local system (lines 3-7). The algorithm then updates the battery levels based on basic energy consumption and broadcast-related energy costs using Equation \ref{eq:payload}. Subsequently, the received instances are batched together (line 8), and the reservoir undergoes an update using a damped window mechanism, considering factors like damping factor, reservoir size, and utility constraints. Following the reservoir update (line 10), the algorithm employs trust patterns to determine the operational status (active or passive) of each node. If a node has sufficient frequency in the reservoir, indicating trustworthiness (frequency $\geq 2$, because it has probably two neighbors), it is set to passive; otherwise, it remains active (lines 12-15). The algorithm ensures that nodes with zero battery levels are marked as "OFF" (line 16). In the case where the system is in an idle state with an empty batch at time \timestamp (line 18-24), the algorithm wakes up the passive nodes, setting them to an active state. The loop continues at each timestamp, dynamically adapting the network device statuses based on energy considerations and trust patterns in the updated reservoir of size \reservoirSize.

Interestingly, the complexity of Algorithm \ref{alg:optimistic_shepherd} is relatively the same that of Algorithm \ref{alg:spasx} after the broadcast phase. In that case, the complexity of processing the batch and the decision making at a time \timestamp is $\complexity(\myalgodampedwindow)+\complexity(\card{\vertices_\timestamp})$. 

\subsection{Evaluation metrics}

The accuracy function and its use aim to evaluate the performance of the network based on the distribution of active and passive nodes, taking into account coverage and non-redundancy aspects. Let's formalize the accuracy mathematically.


\noindent \textbf{Intuition and Motivation:}
\begin{itemize}
	\item \textbf{Coverage:} Denoted by $\coverage(\vertex, \timestamp)$, it measures how many passive nodes are covered by an active node \vertex at time \timestamp. A higher coverage indicates a more effective utilization of active nodes to cover passive nodes. By considering the average number of active nodes covering passive nodes, we aim to assess how well the network is utilizing its active nodes to reach passive nodes. Formally, it is defined as follows:
	
	
	\begin{equation}
		\coverage(\vertex, \timestamp) = \left\{ \begin{array}{cl}
			1  & \text{if} \card{\neighbors(\vertex, \timestamp)}=0 \\
			\frac{\card{\{\vertex' ~:~ \vertex' \in \neighbors(\vertex, \timestamp) \cap \passiveNodes_\timestamp\}}}{\card{\neighbors(\vertex, \timestamp)}} & \text{otherwise.}
		\end{array} \right.
	\end{equation}
	
	\item \textbf{Uniqueness:} Denoted by $\uniqueness(\vertex, \timestamp)$, it measures the non-redundancy of passive node \vertex covered by active nodes at time \timestamp. A higher uniqueness indicates that the covered passive nodes are distinct and not redundant. It takes into account the diversity and non-redundancy of the covered passive nodes. It penalizes redundancy and encourages diversity in the coverage. Formally, it is defined as follows:
	
	
	\begin{equation}
		\uniqueness(\vertex, \timestamp) = \left\{ \begin{array}{cl}
			0  & \text{if} \card{\neighbors(\vertex, \timestamp)}=0 \\
			1 - \frac{\card{\{\vertex' ~:~ \vertex' \in \neighbors(\vertex, \timestamp) \cap \activeNodes_\timestamp\}}-1}{\card{\neighbors(\vertex, \timestamp)}} & \text{otherwise.}
		\end{array} \right.
	\end{equation}
	
	\item \textbf{Safety of the network $\dynaGraph(\vertices_\timestamp, \edges_\timestamp)$:} Denoted by $\safety(\dynaGraph_\timestamp, \timestamp)$, it is a balanced combination of coverage and uniqueness providing an overall measure of the network effectiveness at time \timestamp. The use of the harmonic mean ensures that both aspects contribute meaningfully to the overall evaluation. A higher safety indicates a more efficient and diverse use of active nodes. Formally, it is defined as follows:
	
	$$\safety(\dynaGraph_\timestamp, \timestamp) = \frac{2 \times \left( \sum_{\vertex \in \activeNodes_\timestamp} \coverage(\vertex, \timestamp)\right) \times \left(\sum_{\vertex \in \passiveNodes_\timestamp} \uniqueness(\vertex, \timestamp) \right) }{\left(\card{\passiveNodes_\timestamp}\sum_{\vertex \in \activeNodes_\timestamp} \coverage(\vertex, \timestamp)\right) + \left(\card{\activeNodes_\timestamp}\sum_{\vertex \in \passiveNodes_\timestamp} \uniqueness(\vertex, \timestamp)\right)}.$$
\end{itemize}

